A Probabilistic Framework for Location Inference from Social Media

We study the extent to which we can infer users' geographical locations from social media. Location inference from social media can benefit many applications, such as disaster management, targeted advertising, and news content tailoring. The challenges, however, lie in the limited amount of labeled data and the large scale of social networks. In this paper, we formalize the problem of inferring location from social media into a semi-supervised factor graph model (SSFGM). The model provides a probabilistic framework in which various sources of information (e.g., content and social network) can be combined together. We design a two-layer neural network to learn feature representations, and incorporate the learned latent features into SSFGM. To deal with the large-scale problem, we propose a Two-Chain Sampling (TCS) algorithm to learn SSFGM. The algorithm achieves a good trade-off between accuracy and efficiency. Experiments on Twitter and Weibo show that the proposed TCS algorithm for SSFGM can substantially improve the inference accuracy over several state-of-the-art methods. More importantly, TCS achieves over 100x speedup comparing with traditional propagation-based methods (e.g., loopy belief propagation).

==> problem.tex <==
\section{Problem Definition}
\label{sec:problem} 
In our work, we formalize the geo-location inference problem as a classification problem. For each user, we aim to classify which country/state/city the user comes from. In the real world, some users who turn on the geo-tagging functionality on their mobile phones can be directly labeled by their location. So we can define Twitter network -- the input of our problem -- as a \textit{partially labeled network}.

\begin{definition}{\textbf{\textit{Partially labeled network}}.}
A \textit{partially labeled network} is an augmented social network denoted as $G=(V, E, Y^L, \mathbf{X})$, where $V = V^L \cup V^U$ denote the user set, $V^L$ is the set of labeled users and $V^U$ is the set of unlabeled users; $E \subseteq V\times V$ is the set of relationships between users; $Y^L$ is the set of labels (locations) corresponding to the users in $V^L$; $\textbf{X}$ is the feature matrix associated with users in $V$ where each row represents a user, each column represents a feature, and $x_{ij}$ denotes the value of $j^{th}$ feature of user $v_i$.
\end{definition}

Based on the above definition, we can define the problem of inferring user locations. Given a partially labeled social network, the goal is to infer the locations of all unknown users in the network. More precisely,

\begin{problem}{\textbf{\textit{User geo-location inference}}.} 
Given a \textit{partially labeled network} $G=(V, E, Y^L, \mathbf{X})$, the objective is to learn a classification function
\begin{equation}
f: G=(V, E, Y^L, \mathbf{X}) \rightarrow Y^U
\end{equation}
where $Y^U$ is the set of predicted locations for unlabeled users. 
\end{problem}

Our formulation of user location inference is different from all the previous work we have discussed in Section \ref{sec:related}. We formalize the problem as a semi-supervised learning problem, and we combine both user attributes and social network information into location inference. Our formulation is closer to the real-world scenario, where there are part of labeled users and we want to infer the other users. Traditional methods are usually supervised learning, which only consider labeled data. In Twitter, only fewer than 0.5\% users are geo-labeled. Semi-supervised learning leverages unlabeled data to improve the performance. 


==> related.tex <==
\section{Related Work}
\label{sec:related}

%\reminder{Jie or Yujie}


\begin{table*}[t]
\centering
\caption{\label{related} Characteristics of previous studies of geolocation inference of tweets or Twitter users.}
\small
\begin{tabular}{|c|>{\centering}m{1.4in}|c|c|c|c|}
\hline
\textbf{Authors} & \textbf{Features} & \textbf{Scope} & \textbf{Language} & \textbf{Granularity} & \textbf{Object} \\\hline
Eisenstein et al. \cite{eisenstein2010latent} & Tweet content & US only & All & Coordinate & User  \\\hline
Cheng et al. \cite{cheng2010you} & Tweet content & US only & English & Coordinate & User \\\hline
Ikawa et al. \cite{ikawa2012location} & Tweet content & Japan & English, Japanese & Coordinate & Tweet \\\hline
Ryoo et al. \cite{ryoo2014inferring} & Tweet content & Korea & Korean & Coordinate & User \\\hline
Wing et al. \cite{wing2011simple} & Tweet content & US only & English & Grid cell & User \\\hline
Chen et al. \cite{chen2013interest} & Tweet content & Beijing & Chinese & Coordinate & Tweet \\\hline
Li et al. \cite{li2012towards} & Tweet content + Social network &  US only & English & Coordinate & User \\\hline
Jurgens \cite{jurgens2013s} & Social network & World & All & Coordinate & User \\\hline
Zubiaga et al. \cite{zubiaga2016towards} & Tweet + User profile & World & All & Country & Tweet \\\hline\hline
Present work & Tweet content +  User profile + Social network & World & All & Country & User \\\hline
\end{tabular}
\end{table*}

The location inference problem has been studied by many researchers. Ajao et al. conduct a survey on existing techniques of location inference on Twitter. As well as numerous different techniques, researchers have focused on different settings and pursued different objectives when conducting experiments. Table \ref{related} lists the summary of the previous work, outlining the features, the geographic scope, the languages, the classification granularity, and whether tweet-level or user-level prediction in these studies. 

Most of the previous studies focused on tweet content. Eisenstein et al. \cite{eisenstein2010latent} proposed the Geographic Topic Model to predict user's geolocation from raw text. Cheng et al. \cite{cheng2010you} utilized a probabilistic framework and illustrated how to find local words and overcome tweet sparsity. Ryoo et al. \cite{ryoo2014inferring} used similar idea and applied in Korean data. Ikawa et al. \cite{ikawa2012location} used a rule-based approach to predict the user's current location based on former tweets. Wing et al. \cite{wing2011simple} used language model and information retrieval approach for location estimation.  Chen et al. \cite{chen2013interest} used topic model to determine user's interests and mapped interests to location.  We find all these previous works conducted experiments in a specific region, which is the major limitation of their models. When we want to locate users all around world, these models have difficulty solving the problems such as various languages and too large corpus. Besides, using tweet content to infer the location is not very reliable, because the user can tweet everything they like, not necessarily related to the location.

Jurgens \cite{jurgens2013s} tried to use social network to predict the user location. They used Label Propagation to predict unlabeled users according to their distance to labeled users, but this method did not consider other information. Li et al. \cite{li2012towards} proposed a unified discriminative influence model and utilized both tweet content and social network to predict the user location. However, they focused on US users and tweets written in English only.

Recently, Zubiaga et al. \cite{zubiaga2016towards} studied the problem of inferring country-level location of a tweet, which is the most similar on with our problem. They extracted indicate features from user profile, and trained a SVM to classify tweets to different countries. 

In our work, we want to combine user attributes and social network to infer the user locations. Incorporating social network can infer the location better than singly looking at each user. Our method is effective as well as general that can be extended to solve other inference problems such as inferring gender, age, and education level. The Factor Graph Model in our method has previously been used in tasks such as infer demographics \cite{dong2014inferring} and social ties \cite{tang2011learning}.\reminder{Binxuan: Since FGM has been used in demographics inference, what's the mojor difference and contribution of your model? I see you talked the difference in section 3, but maybe using one more sentence here would be better.}
 
 
